Parallelizing Training of Deep Generative Models on Massive Scientific Datasets

Training deep neural networks on large scientific data is a challenging task that requires enormous compute power, especially if no pre-trained models exist to initialize the process. We present a novel tournament method to train traditional as well as generative adversarial networks built on LBANN, a scalable deep learning framework optimized for HPC systems. LBANN combines multiple levels of parallelism and exploits some of the worlds largest supercomputers. We demonstrate our framework by creating a complex predictive model based on multi-variate data from high-energy-density physics containing hundreds of millions of images and hundreds of millions of scalar values derived from tens of millions of simulations of inertial confinement fusion. Our approach combines an HPC workflow and extends LBANN with optimized data ingestion and the new tournament-style training algorithm to produce a scalable neural network architecture using a CORAL-class supercomputer. Experimental results show that 64 trainers (1024 GPUs) achieve a speedup of 70.2 over a single trainer (16 GPUs) baseline, and an effective 109% parallel efficiency.

==> related_work.tex <==
\section{Related Work}
\label{sec:related}
Recent successes of deep learning in many application domains have
encouraged renewed interest in understanding and optimizing neural
networks. Of particular interest and related to our work is the
subject of scaling neural network training on different architectural
platforms. Distributed and parallel training of deep learning
algorithms is well-studied but mostly focused on the traditional
fields of computer vision and speech recognition
~\cite{tensorflow2015-whitepaper},~\cite{strom2015scalable},~\cite{le2012building},~\cite{dean2012large}.
~\cite{recht2011hogwild,coates2013deep},
~\cite{iandola2015firecaffe},~\cite{goyal2017accurate,keskar2017large,cho2017}. Data and
model parallelism in these work are orthogonal to our work and are used within each
trainer to maximize parallelism. Here, we leverage ideas from these existing domains but focus on 
generative surrogate model for fusion science application and target HPC systems. 


The LTFB algorithm was initially proposed in~\cite{Jacobs2017} and
demonstrates modest scaling on image classification benchmarks.  At
about the same time, researchers at Google Deepmind explored a similar idea for
hyperparameter exploration without data
partitioning~\cite{DBLP:journals/corr/abs-1711-09846}. Deepmind's
work did not address scaling but demonstrate the utility of population-based 
training approaches for hyperparameter optimization on a number of computer vision and
reinforcement learning benchmarks.  
In this work we present new methods for applying these tournmanet methods to
generative adversarial networks, extend them to a
different (scientific) domain with multivariate data, and provide a primary focus on large scale
training using HPC systems.

Scientific machine learning is drawing attention to problems that are beyond
computer vision and natural language processing \cite{spears-deeplearning,
DBLP:journals/corr/KarpatneAFSBGSS16}. %Given that scientific machine (deep) learning is at its infancy,
%there are not many large-scale training of scientific dataset.
Prominent recent works are: exascale deep learning for climate
analytics ~\cite{kurth2018exascale}, and $CosmoFlow$ that used deep learning to learn the universe
at scale ~\cite{mathuriya2018cosmoflow}.  In both
cases, straight forward large-batch data parallelism is used without
addressing convergence issues or the quality of trained regression
network

The climate analytics and cosmology problems mentioned above emphasize the
challenges of data ingestion and present
novel opportunities to improve performance. Kurth et al.~\cite{kurth2018exascale}
developed distributed data staging system in which each rank first
copies a disjoint subset of the entire dataset from the parallel file system
into its fast local storage, and then distributes the files to other ranks that
require them using the point-to-point MPI communication.
This significantly reduces the I/O bottleneck at the filesystem.
However, as the data staging precedes training, each rank needs to hold all the
data files it needs to access on the local storage.
On the other hand, LBANN offers a built-in, in-memory data store in which sample
data are transferred from the owner rank to the consumer rank as needed before
every minibatch using non-blocking communication.
This eliminates the redundant in-memory copies of data, hides the overhead in
redistributing them and reduces the volume of the redistribution
in case that each data file contains multiple samples.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Parallelizing_Training_CycleGAN"
%%% End:

